Low-Rate Overuse Flow Tracer (LOFT): An Efficient and Scalable Algorithm for Detecting Overuse Flows

Current probabilistic flow-size monitoring can only detect heavy hitters (e.g., flows utilizing 10 times their permitted bandwidth), but cannot detect smaller overuse (e.g., flows utilizing 50-100% more than their permitted bandwidth). Thus, these systems lack accuracy in the challenging environment of high-throughput packet processing, where fast-memory resources are scarce. Nevertheless, many applications rely on accurate flow-size estimation, e.g. for network monitoring, anomaly detection and Quality of Service. We design, analyze, implement, and evaluate LOFT, a new approach for efficiently detecting overuse flows that achieves dramatically better properties than prior work. LOFT can detect 1.5x overuse flows in one second, whereas prior approaches fail to detect 2x overuse flows within a timeout of 300 seconds. We demonstrate LOFT's suitability for high-speed packet processing with implementations in the DPDK framework and on an FPGA.

==> sec/outline.tex <==
% - Overuse flow detection is important.

The problem of detecting misbehaving network flows that overuse their
allocated bandwidth has received significant attention since the
seminal paper by Estan and Varghese in 2003~\cite{Estan03}. It remains
an important topic to this date due to the increasing need of latency
sensitive applications, the impact of volumetric DDoS
attacks~\cite{Antonakakis2017}, and the emergence of bandwidth
allocation schemes~\cite{BRSPZHKU2016,LiJiHuBa2016,LeKaGl2013}.


% - Overuse flow detection needs to be done quickly, without keeping per flow state.

The missing piece in realizing guaranteed network performance and DDoS
protection mechanisms is the viable and rapid detection of overuse
flows on Internet \emph{core routers}, which typically have an
aggregate capacity of several Terabits per second (Tbps). However, due
to the high-speed packet processing requirement (e.g., on the order of
100ns per packet), existing approaches for per-flow resource
accounting are either too expensive or too inaccurate to perform:
Keeping flow information on DRAM (whose access latencies over 60ns on
current hardware~\cite{skylake-characteristics,DRAM-latency-2016})
would not suffice the speed requirement, whereas the high cost of fast
memory (e.g., SRAM) prohibits its use for per-flow storage.

%% Currently proposed accurate detection schemes, such as Cisco
%% Netflow / IETF IPFIX~\cite{rfc7011} or EARDet~\cite{Wu14} require
%% memory size on the order of the number of active network flows.


To reduce fast memory usage, an interesting line of research work
devises \emph{shared-counter approaches} that map multiple flows to
the same counter and estimate each flow's \emph{size} based on the
values of the corresponding counters~\cite{Estan03}. Flows with an
estimated size that exceed a pre-defined threshold are considered
malicious. Unfortunately, these approaches suffer from a high number
of false negatives for \emph{low-ratio} overuse flows, or overuse flows
that send close (e.g., 2x) to their permitted limits.

%% non-egregious
%% which means that unless a flow sends at a rate of 100--1000 fold the
%% permitted bandwidth, it will most likely not be detected.

We observe that prior shared-counter approaches fail to accurately
detect low-ratio overuse flows due to high variances of the flow-size
estimators. The variances are mainly caused by 1) the uneven number of
flows across counters, and 2) the uneven flow-size distribution within
the same counter.

%% Another key insight we have about overuse flow detection is that
%% estimating the flow size is an overkill; estimating \emph{flow rank}
%% is sufficient for detecting overuse flows.

To achieve a viable approach that detect low-rate overuse flows with
high probability, we propose \name with two novel techniques to reduce
variances, thereby dramatically imporving over previous
proposals. First, to smooth out the unevenness across counters, \name
counts how many flows fall into a bucket and divides the counter value
by the number of flows. Second, to smooth out the unevenness within a
counter, \name re-groups flows \emph{over time} (in a sequence of
trials) and aggregates the estimators in different trials. By
spreading counters over time, \name is able to keep old counter values
in DRAM and fully utilize SRAM in each trial, allowing the estimator
to converge rapidly to its expectation value. Notice that \name
estimates each flow's \emph{rank}, instead of size, and we show in our
theorectical analysis that rank estimation is sufficient for
accurately detecting overuse flows.

%% \name constructs a hybrid SRAM-DRAM data structure in which only
%% the counters of the current trial are stored in SRAM for online
%% line-rate update, and the counters of past trials are stored in
%% DRAM for offline processing.

%% - 2) DRAM vs.SRAM; using more layers is helpful for CROFT; prior work
%% didn't think about putting counters into DRAM for offline processing;
%% the cost can be amortized over time.

%% - Time division; multi-layer counters spread over time, not
%% space. Prior work didn't think about this. Note that FMF can also
%% benefit from re-grouping; However, for FMF to detect low-rate
%% flows, FMF needs to use many many layers.

Our evaluation using both real and synthetic traffic traces shows
that \name achieves dramatically better properties than prior
work. \name can reliably detect 1.5x overuse flows in one second,
whereas prior approaches fail to detect 8x or less overuse flows with
high probability. We also provide theoretical analysis to guide
parameter selection.

This paper makes the following contributions:
\begin{itemize}
\item We point out that previous shared-counter algorithms are inadequate 
in detecting low-ratio overuse flows due to high variances in their
flow-size estimators.
\item We propose a novel algorithm called \name that computes flow-rank
estimators with low variances. This is achieved by counting the number
of flows falling into a bucket and re-grouping flows over time.

%% lack of counting how many flows fall into a bucket as the reason for a
%% high false negative rate and the fact that only flows that send
%% 100--1000 times the permitted rate can be detected with high
%% confidence.
%% \item We identify that flow size variance within a bandwidth class is
%% an important consideration for overuse flow detection algorithms.
%% Previous algorithms worked well in environments with high flow size
%% variance. In QoS settings, the flow size variance may be low, which
%% further limits the value of previously proposed algorithms.

\item We implement and evaluate \name to confirm that \name is
viable to execute on core routers with Tbps link speeds and can
rapidly detect overuse flows. In addition, \name can handle settings
with small bandwidth variance and where overuse flows only send 50\%
more than their permitted bandwidth.
\item We provide a theoretical analysis to guide the parameter selection of \name. 
\end{itemize}



